Adaptive Inference-Time Scaling via Cyclic Diffusion Search

Diffusion models have demonstrated strong generative capabilities across domains ranging from image synthesis to complex reasoning tasks. However, most inference-time scaling methods rely on fixed denoising schedules, limiting their ability to allocate computation based on instance difficulty or task-specific demands adaptively. We introduce the challenge of adaptive inference-time scaling-dynamically adjusting computational effort during inference-and propose Adaptive Bi-directional Cyclic Diffusion (ABCD), a flexible, search-based inference framework. ABCD refines outputs through bi-directional diffusion cycles while adaptively controlling exploration depth and termination. It comprises three components: Cyclic Diffusion Search, Automatic Exploration-Exploitation Balancing, and Adaptive Thinking Time. Experiments show that ABCD improves performance across diverse tasks while maintaining computational efficiency.

==> Algorithm/pseudo_algo_adaptiveGB.tex <==
\begin{algorithm}[t]
\caption{Adaptive Diffusion Thinker with Adaptive GoBack Sampling}
\label{alg:adaptive-thinking}
\begin{algorithmic}[1]
\Procedure{AdaptiveThinking}{verifier, $T$, $N$, $\texttt{jump}$, $\texttt{GoBackCandidates}$, $\texttt{max\_iter}$, $\texttt{sf}$}
    \State Initialize $particles$:  $\{x_T^{(i)}\}_{i=1}^{N} \sim \mathcal{N}(0, I)$
    \State $\{x_0^{(i)}\}_{i=1}^{N} \gets$ \textsc{JumpyDenoise}($particles$, $\texttt{jump}$) \Comment{denoise until $t=0$ using jumpy DDIM}
    \State $\texttt{GoBackDist} \gets$ Uniform over $\texttt{GoBackCandidates}$ 
    \State $\texttt{GoBackList} \sim \texttt{GoBackDist}$ of size $K$

    \While{$iter < \texttt{max\_iter}$}
        %\State Sample $\texttt{GoBackList} \sim \texttt{GoBackDist}$
        \State $GBparticles \gets \emptyset$

        \For{$t_g \in \texttt{GoBackList}$}
            \State $\{x_{t_g}^{(i)}\}_{i=1}^{N} \gets$ \textsc{Renoise}($\{x_0^{(i)}\}_{i=1}^{N}, t_g$) \Comment{renoise until $t=t_g$}
            \State $GBparticles \gets GBparticles \cup \{x_{t_g}^{(i)}\}_{i=1}^{N}$
        \EndFor

        \State $\{\{x_{0 \gets t_g}^{(i)}\}_{i=1}^{N}\}_{t_g \in \texttt{GoBackList}} \gets$\textsc{JumpyDenoise}($GBparticles$, $\texttt{jump}$)
        \State $rewards \gets$ verifier($\{\{x_{0 \gets t_g}^{(i)}\}_{i=1}^{N}\}_{t_g \in \texttt{GoBackList}}$) \\ \Comment{evaluate all particles from different GB}
        \State $\{\tilde{x}_0^{(i)}\}_{i=1}^{N} \gets$ \textsc{Select} top-$N$ by $rewards$
        \State $sources \gets$ GoBack index $t_g$ of top-$N$ particles

        \State \textbf{// Track reward per $t_g$}
        \For{$g \in \texttt{GoBackList}$}
            \State $R[g] \gets$ mean reward of particles $\{x_{0 \gets t_g}^{(i)}\}_{i=1}^{N}$ from $t_g$
        \EndFor
        \State \textbf{// add exploration term $\epsilon$ for each $t_g$}
        \State $\texttt{GoBackDist} \gets$ Normalize($R + \epsilon$) \Comment{e.g. softmax or normalized weights}
        \State $\texttt{GoBackList} \sim \texttt{GoBackDist}$ of size $K$ \Comment{Sample next GB set proportional to $R[g]$}
        \If{All($sources == 0$) for consecutive $\texttt{sf}$ steps}
            \State \textbf{break While}
        \EndIf

        \State $\{x_0^{(i)}\}_{i=1}^{N} \gets \{\tilde{x}_0^{(i)}\}_{i=1}^{N}$
    \EndWhile
    \State \Return Final $x_0$
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> Algorithm/pseudo_algo_adaptiveThinking.tex <==
\begin{algorithm}[t]
\caption{Adaptive Diffusion Thinker with Adative Thinking Time}
\label{alg:adaptive-thinking}
\begin{algorithmic}[1]
\Procedure{AdaptiveThinking}{verifier, $T$, $N$, $\texttt{jump}$, $\texttt{GoBackList}$, $\texttt{max\_iter}$, $\texttt{sf}$}
    \State Initialize $particles$:  $\{x_T^{(i)}\}_{i=1}^{N} \sim \mathcal{N}(0, I)$
    \State $\{x_0^{(i)}\}_{i=1}^{N} \gets$ \textsc{JumpyDenoise}($particles$, $\texttt{jump}$) \Comment{denoise until $t=0$ using jumpy DDIM}
    \State $iter \gets 0$
    \While{$iter < \texttt{max\_iter}$}
        \State $GBparticles \gets \emptyset$
        \For{$g \in \texttt{GoBackList}$}
            \State $t_g \gets \min(0 + g, T)$
            \State $\{x_{t_g}^{(i)}\}_{i=1}^{N} \gets \textsc{Renoise}(\{x_0^{(i)}\}_{i=1}^{N}, t_g)$ \Comment{renoise until $t=t_g$}
            \State $GBparticles \gets GBparticles \ \cup$ $\{x_{t_g}^{(i)}\}_{i=1}^{N}$
        \EndFor
        \State $\{\{x_{0 \gets t_g}^{(i)}\}_{i=1}^{N}\}_{t_g \in \texttt{GoBackList}} \gets$ \textsc{JumpyDenoise}($GBparticles$, $\texttt{jump}$)
        
        \State $rewards \gets$ verifier($\{\{x_{0 \gets t_g}^{(i)}\}_{i=1}^{N}\}_{t_g \in \texttt{GoBackList}}$) \\ \Comment{evaluate all particles from different GB}
        \State $\{\tilde{x}_0^{(i)}\}_{i=1}^{N} \gets$ \textsc{Select} top-$N$ particles by $rewards$
        \State $sources \gets$ GoBack index $t_g$ of top-$N$ particles
        \If{All($sources == 0$) for consecutive steps \texttt{sf}}
        \State \textbf{break While}
        \EndIf
        \State $iter \gets iter + 1$
        \State $\{x_0^{(i)}\}_{i=1}^{N} \gets \{\tilde{x}_0^{(i)}\}_{i=1}^{N}$
    \EndWhile
    \State \Return Final $x_0$
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> Algorithm/pseudocode_Simpler.tex <==
\begin{comment}
\begin{algorithm}[t]
\caption{ABCD: Adaptive Bi-directional Cyclic Diffusion}
\label{alg:adaptive-thinking}
\begin{algorithmic}[1]
\Procedure{ABCD}{\texttt{verifier}, $T$, $\mathcal{T}$, \texttt{max\_iter}, $\kappa$}%\texttt{GoBackList},\texttt{stop\_flag}
    \State Initialize $K$ particles $\{x_T^{(i)}\}$ from $\cN(0, I)$
    \State Denoise to obtain $\{x_0^{(i)}\}$ via Fast denoising
    \While{less than \texttt{max\_iter}}
        \State Re-noise $\{x_0^{(i)}\}$ to each $t_g \in$  $\mathcal{T}$
        \State Jumpy Denoise again from each $t_g$ to get new $\smash{\{x_0^{(i)}\}}$
        \State Evaluate all candidates reward $r(\cdot)$ using \texttt{verifier}
        \State Select top-$K$ particles across all $t_g$ by reward
        \State \textbf{If} Selected top-$K$ particles come from smallest $t_g$ for $\kappa$ times consecutively
        \State \quad \textbf{break} %\Comment{adaptive terminal condition}
    \EndWhile
    \State \Return Select Best particle from top-$K$ particles %$\arg \max_{x_{1...N}}$ $r(x_0^{(i)})$
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{comment}

\begin{algorithm}[t]
\caption{ABCD: Adaptive Bi-directional Cyclic Diffusion}
\label{alg:adaptive-thinking}
\begin{algorithmic}[1]
\Procedure{ABCD}{\texttt{verifier}, $T$, $\mathcal{T}$, \texttt{max\_iter}, $\kappa$}%\texttt{GoBackList},\texttt{stop\_flag}
    \State Initialize $K$ particles $\{x_T^{(i)}\}$ from $\cN(0, I)$
    \State Denoise to obtain $\{x_0^{(i)}\}$ via Fast denoising
    \While{cycle less than \texttt{max\_iter}}
        \State Re-noise $\{x_0^{(i)}\}$ to each $t_g \in$  $\mathcal{T}$
        \State Jumpy Denoise again from each $t_g$ to get new $\smash{\{x_0^{(i)}\}}$
        \State Evaluate all candidates reward $r(\cdot)$ using \texttt{verifier}
        \State Select top-$K$ particles across all $t_g$ by reward
        \State \textbf{If} Selected top-$K$ particles come from smallest $t_g$ for $\kappa$ times consecutively
        \State \quad \textbf{break} %\Comment{adaptive terminal condition}
    \EndWhile
    \State \Return Select Best particle from top-$K$ particles %$\arg \max_{x_{1...N}}$ $r(x_0^{(i)})$
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> Figures_tex/MoG_D2_21_81.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]
    {Figures/MoG_comparison.png}
    \caption{
    \textbf{Particle updates across cycles on MoG Dataset 2.}
     All instances begin from an initial incorrect prediction, requiring additional correction during inference. GB=21 fails to escape the initial cluster of modes, whereas GB=81 enables transitions across regions but refines inefficiently. Our method combines coarse transitions to explore distant regions and fine adjustments for local refinement, enabling faster and more effective inference time adjustment.
    }
    \label{fig:MoG_D2_21_81}
\end{figure}

==> Figures_tex/OGBenchMazeGiant.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\linewidth]{Figures/OGBenchMazeGiant_with_baseline.png}
    \caption{\textbf{OGBench PointMaze Giant results.}}
    \label{fig:myplot}
\end{figure}

==> Figures_tex/OGBenchMazeGiant_ablation_termination_percentage.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/OGBenchMazeGiant_ablation_termination_percentage.png}
    \caption{How termination percentage influence the performance of the model: lower thresholds save the compute but risk premature termination.}
    \label{fig:Ablation terminatino percentage}
\end{figure}


==> Figures_tex/OGBenchMazeGiant_multiGB_tex.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/OGBenchMazeGiant_multiple_GB.png}
    \caption{Different Go Back step sizes in maze}
    \label{fig:Different GB}
\end{figure}


==> Figures_tex/OGBenchMazeGiant_visualization.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/OGBenchMazeGiant_visualization.png}
    \caption{Visualization of the generated plans across iteration until the first successful execution, comparing Single Go Back step size versus Multiple Go Back step size. We observe that Multiple Go Back step size requires fewer iterations than any individual single Go Back step size.}
    \label{fig:myplot}
\end{figure}

==> Figures_tex/OGBenchMazeGiant_with_baseline_tex.tex <==
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{Figures/OGBenchMazeGiant_with_baseline_same_particle.png}
%     \caption{Comparison with other particle-based method given the same number of particles}
% \end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/OGBenchMazeGiant_with_baseline.png}
    \caption{Comparison with other particle-based method preserved their nature}
\end{figure}

==> Figures_tex/OGBenchMazeLarge.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\linewidth]{Figures/OGBenchMazeLarge_with_baseline.png}
    \caption{\textbf{OGBench PointMaze Large results.}}
    \label{fig:myplot}
\end{figure}

==> Figures_tex/OGBenchMazeLarge_SOP_Failure.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{Figures/OGBenchMazeLarge_SOP_failures.png}
    \caption{Comparison between trajectories generated by Search over Paths and our Adaptive Thinking method.  Adaptive Thinking yields  higher-quality trajectories, while Search over Paths fail to generate decent paths.}
\end{figure}

==> Figures_tex/OGBenchMaze_Giant_Large_aligned.tex <==
\begin{comment}
\begin{wrapfigure}{r}{0.55\textwidth}
    \centering
    \vspace{-7pt}
    % \begin{subfigure}[b]
    % {0.55\textwidth}
        \includegraphics[width=0.55\textwidth]{Figures/OGBenchMaze_Giant_Large_with_baseline.png}
        \label{fig:large}
    % \end{subfigure}
    
    \caption{\textbf{OGBench PointMaze task results.} Success rates across large and giant mazes. Our ABCD approach consistently outperforms baselines, rapidly achieving higher success rates with fewer inference time and attaining perfect performance, particularly in the Giant maze, emphasizing its superior efficiency and effectiveness.}
    \label{fig:ogbench_performance}
\end{wrapfigure}
\end{comment}
% \begin{wrapfigure}{r}{0.42\textwidth}
%     \centering
%     \vspace{-9pt} 
%     \includegraphics[width=\linewidth]{Figures/Sudoku_per_provided.png}
%     \caption{\textbf{Mean accuracy across four difficulty levels}—Very Hard (17-19 provided), Hard (20-21 provided), Medium (22-24 provided), and Easy (25-27 provided).}
%     \vspace{-1em}
%     \label{fig:Sudoku_per_provided}
% \end{wrapfigure}


\begin{figure}{t}{0.55\textwidth}
    \centering
    \vspace{-9pt}
    % \begin{subfigure}[b]
    % {0.55\textwidth}
        \includegraphics[width=0.55\textwidth]{Figures/OGBenchMaze_Giant_Large_with_baseline.png}
        \label{fig:large}
    % \end{subfigure}
    
    \caption{\textbf{OGBench PointMaze task results.} Success rates across large and giant mazes. Our ABCD approach consistently outperforms baselines, rapidly achieving higher success rates with fewer inference time and attaining perfect performance, particularly in the Giant maze, emphasizing its superior efficiency and effectiveness.}
    \label{fig:ogbench_performance}
\end{figure}

==> Figures_tex/OGBench_per_MazeSize_tex.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{Figures/OGBench_diff_MazeSize.png}
    \caption{\textbf{OGBench PointMaze task results.} For fair comparison, inference-time computation for each method was scaled along its respective core controllable axis. Our ABCD approach consistently outperforms baselines, rapidly achieving higher success rates with fewer inference time and attaining perfect performance, particularly in the Giant maze, emphasizing its superior efficiency and effectiveness.}
    \label{fig:myplot}
\end{figure}

\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \input{Figures_tex/OGBenchMazeGiant}
    \caption{Giant maze}
    \label{fig:maze-giant}
  \end{subfigure}\hfill
  \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \input{Figures_tex/OGBenchMazeLarge}
    \caption{Large maze}
    \label{fig:maze-large}
  \end{subfigure}
  \caption{Side-by-side comparison of OGBench PointMaze sizes.}
  \label{fig:mazes}
\end{figure}

==> Figures_tex/PM_Mol_comparison.tex <==
\begin{comment}
\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\linewidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/PixelMaze_comparison_15.png}
        \caption{
        Comparing with the baseline in Pixel Maze datset. Models are trained on smaller mazes (sizes 4$\sim$6) and tested on larger ones.
        }
        \label{fig:sudoku_comparison_full}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/Molecular_comparison.png}
        \caption{Comparing with the baseline in QM9 continuous 3D structure prediction task task.}
        \label{fig:PixelMaze_comparison}
    \end{minipage}
\end{figure}
\end{comment}
\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.48\linewidth}
        \vspace{0pt} 
        \centering
        \includegraphics[width=\linewidth]{Figures/PixelMaze_comparison_15.png}
        \caption{
        \textbf{Pixel maze path finding result.}
        Success rate (\%) on the OOD Pixel Maze size-15 test set. For each method, inference-time computation was scaled as much as possible along its core controllable axis to ensure a fair comparison under expanded budgets.
        }
        \label{fig:sudoku_comparison_full}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\linewidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{Figures/Molecular_comparison.png}
        \caption{
        \textbf{Molecular 3D structure prediction task Result.}
        Molecular Stability rate (\%) on the QM9 dataset. For each method, inference-time computation was scaled as much as possible along its core controllable axis to ensure a fair comparison under expanded budgets. \gb{TODO, need detail}.}
        \label{fig:Molecular_comparison}
    \end{minipage}
\end{figure}

==> Figures_tex/PixelMaze_adaptive.tex <==
\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/PixelMaze_adaptive.png}
    \caption{Comparison between Search over Paths and Ours in Maze Size 15 in PixelMaze.}
    \label{fig:myplot}
\end{figure}

% right plot left explanation
\begin{figure}[H]
    \centering
    \begin{minipage}[t]{0.5\textwidth}
        \vspace{0pt}
        \textbf{} \gb{TODO}.
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{Figures/PixelMaze_adaptive.png}
        \caption{.}
        \label{fig:sudoku_per_instance}
    \end{minipage}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{minipage}[t]{0.5\textwidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{Figures/PixelMaze_adaptive.png}
        \caption{Comparison of performance against average inference time per sample on Pixel Maze (Size 15). The adaptive terminal condition enables early stopping on easier instances, thereby reducing unnecessary computation. This allows the model to allocate its budget more effectively—spending less time where it isn’t needed and more where it is—leading to faster and more efficient performance improvements under the same overall inference budget.}
        \label{fig:sudoku_per_instance}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
        \vspace{0pt}
        \textbf{} Comparison of performance against average inference time per sample on Pixel Maze (Size 15). The adaptive terminal condition enables early stopping on easier instances, thereby reducing unnecessary computation. This allows the model to allocate its budget more effectively—spending less time where it isn’t needed and more where it is—leading to faster and more efficient performance improvements under the same overall inference budget..
    \end{minipage}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{minipage}[t]{0.38\textwidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{Figures/PixelMaze_adaptive.png}
        \caption{Performance comparison with vs. without adaptive terminal condition in Pixel Maze Size 15. x-axis is the average inference time per sample. %The adaptive terminal condition enables early stopping on easier instances, thereby reducing unnecessary computation.
        }
        \label{fig:pixelmaze_adaptive_comparison}
    \end{minipage}
    \hspace{0.03\textwidth} 
    \begin{minipage}[t]{0.45\textwidth}
        \vspace{0pt}
        %\raggedright  
        Figure~\ref{fig:pixelmaze_adaptive_comparison} illustrates the time-efficiency gains enabled by the adaptive terminal condition, showing how it improves performance relative to average inference time per sample on Pixel Maze (Size 15). Our adaptive terminal condition reduces overthinking by stopping early on easy instances, thus saving unnecessary computation and improving efficiency. This enables the model to spend more time only when needed, achieving faster performance gains under the same overall inference budget. %This allows the model to allocate its budget more effectively—spending less time where it isn’t needed and more where it is—leading to faster and more efficient performance improvements under the same overall inference budget.
    \end{minipage}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[H]
    \centering
    \begin{minipage}[t]{0.55\textwidth}
        \vspace{0pt}
        Figure~\ref{fig:adaptive_comparison} illustrates the time-efficiency gains enabled by the adaptive terminal condition, showing how it improves performance relative to average inference time per sample on Pixel Maze (Size 15). Our adaptive terminal condition reduces overthinking by stopping early on easy instances, thus saving unnecessary computation and improving efficiency. This enables the model to spend more time only when needed, achieving faster performance gains under the same overall inference budget.
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.42\textwidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{Figures/PixelMaze_adaptive.png}
        \caption{Performance comparison with vs. without adaptive terminal condition in Pixel Maze Size 15. x-axis is the average inference time per sample. 
        }
        \label{fig:adaptive_comparison}
    \end{minipage}
\end{figure}
\end{comment}

\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
    \vspace{-10pt} 
    \includegraphics[width=\linewidth]{Figures/PixelMaze_adaptive.png}
    \caption{\textbf{Performance comparison with vs. without adaptive terminal condition in Pixel Maze Size 15.} x-axis is the average inference time per sample.}
     \vspace{-8pt}
    \label{fig:adaptive_comparison}
\end{wrapfigure}




==> Figures_tex/PixelMaze_comparison_baseline_15.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/PixelMaze_comparison_baseline.png}
    \caption{Comparison between Search over Paths and Ours in Maze Size 15 in PixelMaze.}
    \label{fig:myplot}
\end{figure}

==> Figures_tex/PixelMaze_thinking_tex.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/PixelMaze_Thinking_time.png}
        \caption{different thinking time per Maze Size in PixelMaze(11 to 15)}
        \label{fig:sudoku}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/PixelMaze_thinking_iteration.png}
        \caption{different thinking iteration per Maze Size in PixelMaze(11 to 15).}
        \label{fig:tmaze}
    \end{minipage}
\end{figure}

==> Figures_tex/Single_Multi.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Sudoku_Single_Multi.png}
        \caption{Comparing Sinlge Go Back and Mulitple Go Back in Sudoku.}
        \label{fig:sudoku_multi_single}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/PixelMaze_Single_Multi.png}
        \caption{Comparing Sinlge Go Back and Mulitple Go Back in Pixel Maze.}
        \label{fig:pixelmaze_multi_single}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/OGBenchMazeGiant_Single_Multi.png}
        \caption{Comparing Single Go Back and Mulitple Go Back in OGBench Maze.}
        \label{fig:ogbench_multi_single}
    \end{minipage}
\end{figure}

==> Figures_tex/Sudoku_GB30_baseline_tex.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Sudoku_GB30_with_baseline.png}
    \caption{compare Go Back = 30 version with other baseline on Sudoku.}
    \label{fig:myplot}
\end{figure}

==> Figures_tex/Sudoku_comparison_baseline.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{Performance} & \textbf{Inference Time (s)} \\
\midrule
SD & 0.35 $\pm$ 0.1 & 0.28 \\
BoN(N=40) & 0.558 $\pm$ 0.09 & 0.29 \\
FKD & 0.745 $\pm$ 0.1 & 0.32 \\
DLBS & 0.828 $\pm$ 0.09 & 0.5 \\
SoP($\Delta f$=9, $\Delta b$=10) & 0.960 $\pm$ 0.06 & 2.04 \\
ADT(Ours) & \textbf{0.996} $\pm$ \textbf{0.01} & 0.99 \\
\bottomrule
\end{tabular}
\vspace{0.5em}
\caption{This table summarizes the overall results averaged across datasets with 17 to 28 given entities. Our method achieves the highest performance while maintaining lower inference time compared to SoP, demonstrating the efficiency of adaptively allocating computation based on instance difficulty.}
\label{tab:sudoku_table_comparison}
\end{table}

==> Figures_tex/Sudoku_comparison_per_provided.tex <==
\begin{figure}[H]
    \centering
    \begin{minipage}[t]{0.55\textwidth}
        \centering
        \vspace{0pt}
        \includegraphics[width=\linewidth]{Figures/Sudoku_per_provided_baseline.png}
        \caption{Performance comparison with baselines across different numbers of provided digits (17–26) on the Sudoku task.}
        \label{fig:sudoku_bar_comparison}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.4\textwidth}
        \vspace{0pt}
        As shown in Figure~\ref{fig:sudoku_bar_comparison}, our ABCD achieves consistently higher performance across varying difficulty levels, with notably less performance degradation on harder instances (e.g., 17 provided digits). This robustness stems from its ability to allocate more computation to challenging inputs, unlike baseline methods that uniformly apply fixed inference-time budgets. 
    \end{minipage}
\end{figure}

==> Figures_tex/Sudoku_multiGB_tex.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Sudoku_multiple_GB.png}
    \caption{add multiple Go Back version on Sudoku.}
    \label{fig:myplot}
\end{figure}

==> Figures_tex/Sudoku_per_instance.tex <==
\begin{comment}
\begin{figure}[H]
    \centering
    \begin{minipage}[t]{0.42\textwidth}
        \vspace{0pt}
        \textbf{Existence of Inference time scalable go back noise level per instances.} Furthermore, we observe that the optimal noise level can differ even across instances within the same task. Figure~\ref{fig:sudoku_per_instance} shows that in Sudoku, the preferred Go-Back level differs depending on the number of provided entities (e.g., 14 versus 44 provided entities), underscoring the necessity of instance-specific adaptation.
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.55\textwidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{Figures/Sudoku_per_instance.png}
        \caption{Per-instance analysis of inference-time scaling behavior across different Go-Back noise levels.  
        \textbf{Left:} Results for Sudoku instances with 14 provided entities.  
        \textbf{Right:} Results for instances with 44 provided entities.   
        %The optimal noise level differs across instances, highlighting the importance of adaptive scheduling during inference.
        }
        \label{fig:sudoku_per_instance}
    \end{minipage}
\end{figure}
\end{comment}

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    %\vspace{-5pt}
    \includegraphics[width=\linewidth]{Figures/Sudoku_per_instance.png}
    \caption{\textbf{Existence of Inference time scalable go back temperature per instances.} Per-instance analysis of inference-time scaling behavior across different Go-Back temperatures.  
        \textbf{Left:} Results for Sudoku instances with 14 provided entities.  
        \textbf{Right:} Results for instances with 44 provided entities.   }
    \vspace{-4mm}
    \label{fig:Sudoku_per_instance}
\end{wrapfigure}



==> Figures_tex/Sudoku_thinking_tex.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Sudoku_Thinking_Time.png}
        \caption{different thinking time per provided number in Sudoku(17 to 34)}
        \label{fig:sudoku}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Sudoku_Thinking_iteration.png}
        \caption{different thinking iteration per provided number in Sudoku(17 to 34).}
        \label{fig:tmaze}
    \end{minipage}
\end{figure}

==> Figures_tex/Sudoku_version_tex.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Sudoku_adaptiveGB.png}
        \caption{Add adaptive Go Back version on Sudoku.}
        \label{fig:sudoku}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Sudoku_finerGB.png}
        \caption{Add Finer Search Go Back version on Sudoku.}
        \label{fig:tmaze}
    \end{minipage}
\end{figure}

==> Figures_tex/Sudoku_visualization_center.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Visualization_for_Sudoku.png}
    \caption{Visualization of $x_0$ prediction through iteration per four Go Back step size in 22 provided Sudoku Data. We observe that the performance gain from additional iterations is highly sensitive to the choice of Go Back step size..}
    \label{fig:myplot}
\end{figure}



==> Figures_tex/Sudoku_visualize_per_iter_tex.tex <==
\begin{figure}[t]
    \centering

    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=1\linewidth]{Figures/Sudoku_GB10.png}
        \caption{Go Back step size = 10.}
        \label{fig:a}
    \end{subfigure}

    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=1\linewidth]{Figures/Sudoku_GB20.png}
        \caption{Go Back step size =20.}
        \label{fig:b}
    \end{subfigure}

    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=1\linewidth]{Figures/Sudoku_GB30.png}
        \caption{Go Back step size =30.}
        \label{fig:c}
    \end{subfigure}

    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=1\linewidth]{Figures/Sudoku_GB40.png}
        \caption{Go Back step size =40.}
        \label{fig:d}
    \end{subfigure}

    \caption{
        Visualization of $x_0$ prediction through iteration per four Go Back step size in 22 provided Sudoku Data. We observe that the performance gain from additional iterations is highly sensitive to the choice of Go Back step size.
    }
    \label{fig:all_baselines}
\end{figure}

==> Figures_tex/Thinking.tex <==
\begin{comment}
\begin{figure}[H]
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Sudoku_thinking_iteration.png}
        \caption{different thinking assingment per provided number in Sudoku(17 to 34)}
        \label{fig:sudoku_thinking}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/PixelMaze_thinking_iteration.png}
        \caption{different thinking assingment per Maze size in PixelMaze(11 to 15).}
        \label{fig:pixelmaze_thinking}
    \end{minipage}
\end{figure}



\begin{figure}[H]
    \centering
    \begin{minipage}[t]{0.48\textwidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{Figures/Sudoku_thinking_iteration.png}
        \caption{Performance comparison with vs. without adaptive terminal condition in Pixel Maze Size 15. x-axis is the average inference time per sample. %The adaptive terminal condition enables early stopping on easier instances, thereby reducing unnecessary computation.
        }
        \label{fig:pixelmaze_adaptive_comparison}
    \end{minipage}
    \hspace{0.03\textwidth} 
    \begin{minipage}[t]{0.45\textwidth}
        \vspace{0pt}
        %\raggedright  
        Figures~\ref{fig:pixelmaze_adaptive_comparison} shows the resulting thinking iteration counts across different difficulty levels. We observe that stricter stop flag conditions naturally lead to longer thinking times and more iterations. Moreover, the model adaptively allocated more search effort to harder instances—larger mazes and Sudoku puzzles with fewer given numbers—demonstrating that the proposed adaptive termination effectively balances computational effort based on problem complexity.  
    \end{minipage}
\end{figure}
\end{comment}
\begin{comment}
\noindent
\begin{minipage}[t]{0.33\textwidth}
    \vspace{0pt}
    \centering
    \includegraphics[width=\linewidth]{Figures/Sudoku_thinking_iteration.png}
    \captionof{figure}{Performance comparison with vs. without adaptive terminal condition in Pixel Maze Size 15. x-axis indicates average inference time per sample.}
    \label{fig:Sudoku_thinking_iteration}
\end{minipage}%
\hspace{0.03\textwidth}
\begin{minipage}[t]{0.64\textwidth}
    \vspace{0pt}
    Figures~\ref{fig:Sudoku_thinking_iteration} shows the resulting thinking iteration counts across different difficulty levels. We observe that stricter stop flag conditions naturally lead to longer thinking times and more iterations. Moreover, the model adaptively allocated more search effort to harder instances—larger mazes and Sudoku puzzles with fewer given numbers—demonstrating that the proposed adaptive termination effectively balances computational effort based on problem complexity.  
\end{minipage}
\end{comment}

\begin{wrapfigure}{l}{0.4\textwidth}
    \centering
    \vspace{-8pt} 
    \includegraphics[width=\linewidth]{Figures/Sudoku_thinking_iteration.png}
    \caption{Different thinking assignment per hardness in Sudoku (provided Number from 17 to 34).}
    \vspace{-3mm}
    \label{fig:Sudoku_thinking_iteration}
\end{wrapfigure}


==> Figures_tex/comparison.tex <==
\begin{comment}
\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/Sudoku_comparison_full.png}
        \caption{Comparing with the baseline in Sudoku harder datset.}
        \label{fig:sudoku_comparison_full}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/PixelMaze_comparison_15.png}
        \caption{Comparing with the baseline in PixelMaze Size = 15.}
        \label{fig:PixelMaze_comparison}
    \end{minipage}
\end{figure}
\end{comment}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{Figures/Sudoku_comparison_full.png}
        \label{fig:sudoku_comparison_full}
    \end{subfigure}
    \hspace{0.2mm}
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]%{Figures/Sudoku_per_provided_baseline.png}
        {Figures/Sudoku_per_provided.png}
        \label{fig:sudoku_bar_comparison}
    \end{subfigure}
    \caption{\textbf{Sudoku Puzzle Completion Results.} \textbf{Left}: Mean accuracy on Harder dataset (17$\sim$28 entities provided) by giving more computational budget (sec.). \textbf{Right:} Mean accuracy across four difficulty levels—Very Hard (17$\sim$19 provided), Hard (20$\sim$21 provided), Medium (22$\sim$24 provided), and Easy (25$\sim$27 provided)—defined by the number of provided digits. All instances were evaluated within the same test set, and results are grouped post hoc by difficulty for analysis.}
    \label{fig:sudoku_performance}
    \vspace{-5mm}
\end{figure}

==> Figures_tex/per_GB_tex.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Sudoku_per_GB.png}
        \caption{4 different Go Back step sizes in provided Sudoku.}
        \label{fig:sudoku_per_GB}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/PixelMaze_per_GB.png}
        \caption{4 different Go Back step sizes in Pixel Maze (size = 15).}
        \label{fig:pixelmaze_per_GB}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/OGBenchMazeGiant_multiple_GB.png}
        \caption{Different Go Back step sizes in OGBench Maze Giant.}
        \label{fig:ogbench_per_GB}
    \end{minipage}
\end{figure}

==> Figures_tex/sudoku_per_instance.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.48\textwidth}
        \vspace{0pt}
        \small
        Furthermore, we observe that the optimal noise level can differ even across instances within the same task. 
        As shown in the figure, in Sudoku, the preferred Go-Back level differs depending on the number of provided digits (e.g., 14 versus 44 provided entities), underscoring the necessity of instance-specific adaptation.
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{Figures/Sudoku_per_instance.png}
        \caption{Instance-dependent optimal Go-Back noise levels in Sudoku.}
        \label{fig:sudoku_per_instances}
    \end{minipage}
\end{figure}

==> Tables/All_comparison.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\captionsetup{skip=10pt}

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llccc ccc}
\toprule
\textbf{Inference Method} & \textbf{Variant} 
& \multicolumn{3}{c}{\textbf{Maze}} 
& \multicolumn{3}{c}{\textbf{Sudoku}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
& 
& \textbf{Performance} & \textbf{Time} & \textbf{NFE} 
& \textbf{Performance} & \textbf{Time} & \textbf{NFE} \\
\midrule

\multirow{1}{*}{Standard Diffusion} 
  & DDIM baseline &  &  &  &  &  & \\

\midrule

\multirow{3}{*}{Best of N} 
  & N = 40 &  &  &  &  &  & \\
  & N = 80 &  &  &  &  &  & \\
  & N = 120 &  &  &  &  &  & \\

\midrule

\multirow{4}{*}{Search over Paths}
  & $\Delta f$=10, $\Delta b$=5 &  &  &  &  &  & \\
  & $\Delta f$=8, $\Delta b$=4 &  &  &  &  &  & \\
  & $\Delta f$=6, $\Delta b$=3 &  &  &  &  &  & \\
  & $\Delta f$=50, $\Delta b$=25 &  &  &  &  &  & \\

\midrule

\multirow{4}{*}{Go Back} 
  & GB = 10, iter = 55 &  &  &  &  &  & \\
  & GB = 20, iter = 55 &  &  &  &  &  & \\
  & GB = 30, iter = 55 &  &  &  &  &  & \\
  & GB = 40, iter = 55 &  &  &  &  &  & \\

\midrule

\multirow{1}{*}{Multiple Go Back} 
  & iter = 55 &  &  &  &  &  & \\

\midrule

\multirow{1}{*}{Adaptive Go Back} 
  & iter = 55 &  &  &  &  &  & \\

\midrule

\multirow{1}{*}{Adaptive Thinking} 
  & max iter = 100 &  &  &  &  &  & \\

\bottomrule
\end{tabular*}
\caption{Comparison of inference-time strategies on Maze and Sudoku.}
\label{tab:adaptive-diffusion-maze-sudoku}
\end{table}

==> Tables/MoG_single_multi_comparison.tex <==
\begin{table}[H]
\begin{minipage}[t]{0.45\textwidth}
\centering
\scriptsize  
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.3}

\caption{Success rate and distance to goal for Multi Go-Back and fixed Go-Back levels on two Gaussian Mixture datasets.}
\vspace{4pt} 

\begin{tabular}{lcccc}
\toprule
\textbf{Method} 
& \multicolumn{2}{c}{\textbf{Dataset 1}} 
& \multicolumn{2}{c}{\textbf{Dataset 2}} \\
& Success & Distance 
& Success & Distance \\
\midrule
ABCD (Ours) & \textbf{100} & \textbf{0.08 ± 0.03} & \textbf{100} & \textbf{0.03 ± 0.01} \\
GB 21 & 95 & 0.17 ± 0.09 & 26 & 3.97 ± 6.00 \\
GB 41 & 0 & 2.90 ± 0.60 & 59 & 1.73 ± 4.63 \\
GB 61 & 0 & 7.80 ± 0.85 & 7 & 2.94 ± 1.19 \\
GB 81 & 0 & 42.81 ± 6.62 & 0 & 36.46 ± 11.12 \\
\bottomrule
\end{tabular}
\label{tab:gb_comparison}
\end{minipage}
\end{table}

\begin{table}[H]
\begin{minipage}[t]{0.48\textwidth}
\centering
\scriptsize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.3}

\caption{Success rate and mean number of iterations (max 100) for Multi and fixed Go-Back levels on Gaussian Mixture datasets.}
\vspace{4pt}

\begin{tabular}{lcccc}
\toprule
\textbf{Method} 
& \multicolumn{2}{c}{\textbf{Dataset 1}} 
& \multicolumn{2}{c}{\textbf{Dataset 2}} \\
& Success & Mean Iter 
& Success & Mean Iter \\
\midrule
ABCD (Ours) & \textbf{100} & \textbf{3.36} & \textbf{100} & \textbf{7.02} \\
GB 21 & \textbf{100} & \textbf{2.06} & 79 & 16.14 \\
GB 41 & 8 & 46.38 & \textbf{100} & \textbf{6.77} \\
GB 51 & 0 & -- & 100 & 19.66 \\
GB 61 & 0 & -- & 100 & 15.05 \\
GB 81 & 0 & -- & 6 & 43.33 \\
\bottomrule
\end{tabular}
\label{tab:gb_iter_comparison}
\end{minipage}
\end{table}



==> Tables/OGBench_GoBack_comparison.tex <==
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \captionsetup{skip=10pt}  

% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llcccccccccccc}
% \toprule
% \textbf{Method} & \textbf{Variant} & \multicolumn{12}{c}{\textbf{Iterations}} \\
% \cmidrule(lr){3-14}
%  &  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 15 & 20 \\
% \midrule

% \multirow{8}{*}{Go Back}
%   & GB = 32 &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 64 &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 96 &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 128 &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 160 &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 192 &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 224 &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 256 &  &  &  &  &  &  &  &  &  &  &  &  \\


% % \midrule

% % \multirow{3}{*}{Multiple GB}
% %   & 10 even &  &  &  &  &  &  &  &  &  &  &  &  \\
% %   & 5 even &  &  &  &  &  &  &  &  &  &  &  &  \\
% %   & 3 even &  &  &  &  &  &  &  &  &  &  &  &  \\
  
% % \bottomrule


% % \multirow{3}{*}{Adaptive GB}
% %   & 10 even &  &  &  &  &  &  &  &  &  &  &  &  \\
% %   & 5 even &  &  &  &  &  &  &  &  &  &  &  &  \\
% %   & 3 even &  &  &  &  &  &  &  &  &  &  &  &  \\
  
% \bottomrule
% \end{tabular*}
% \caption{Comparison across different Go Back step size and Multiple Go Back step size in OGBench Maze Giant.}
% \label{tab:go-back-vs-iterations}
% \end{table}


% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \captionsetup{skip=10pt}  
% \begin{tabular}{llcccccccccccccccccc}
% \toprule
% \textbf{Method} & \textbf{Variant} & \multicolumn{18}{c}{\textbf{Iterations}} \\
% \cmidrule(lr){3-20}
%  &  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 15 & 20 & 25 & 30 & 35 & 40 & 45 & 50 \\
% \midrule

% \multirow{8}{*}{Go Back}
%   & GB = 32 &  20+/-20 & 20+/-20 & 26+/-20 & 28+/-20 & 26+/-20 & 28+/-22 & 28+/-20 & 26+/-18 & 28+/-20 & 30+/-18 & 32+/-22 & 32+/-22 & 28+/-20 & 36+/-27 & 32+/-18 & 34+/-18 & 36+/-22 & 34+/-24 &  \\
%   & GB = 64 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 96 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 128 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 160 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 192 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 224 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%   & GB = 256 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \bottomrule
% \end{tabular}
% \caption{Comparison across different Go Back step sizes and Multiple Go Back step sizes in OGBench Maze Giant.}
% \label{tab:go-back-vs-iterations}
% \end{table}

% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \captionsetup{skip=10pt}  
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llcccccccccccccccccc}
% \toprule
% \textbf{Method} & \textbf{Variant} & \multicolumn{18}{c}{\textbf{Iterations}} \\
% \cmidrule(lr){3-20}
%  &  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 15 & 20 & 25 & 30 & 35 & 40 & 45 & 50 \\
% \midrule

% \multirow{8}{*}{Go Back}
%   & GB = 32 & 20±20 & 20±20 & 26±20 & 28±20 & 26±20 & 28±22 & 28±20 & 26±18 & 28±20 & 30±18 & 32±22 & 32±22 & 28±20 & 36±27 & 32±18 & 34±18 & 36±22 & 34±24 &  \\
%   & GB = 64 & 20±20 & 24±22 & 24±20 & 30±22 & 32±24 & 30±22 & 36±23 & 32±24 & 36±23 & 32±20 & 38±26 & 36±25 & 38±21 & 34±22 & 38±26 & 36±25 & 38±26 & 34±22 &  \\
%   & GB = 96 & 20±20 & 26±22 & 28±22 & 30±22 & 28±22 & 34±20 & 36±23 & 38±29 & 30±24 & 36±27 & 42±27 & 42±17 & 46±20 & 46±20 & 44±17 & 46±18 & 48±18 & 46±13 &  \\
%   & GB = 128 & 20±18 & 30±26 & 28±20 & 38±26 & 38±21 & 44±28 & 44±20 & 48±18 & 54±22 & 46±22 & 56±17 & 62±21 & 62±21 & 60±20 & 62±21 & 62±21 & 64±17 & 64±20 &  \\
%   & GB = 160 & 26±22 & 42±23 & 50±22 & 62±21 & 58±17 & 60±18 & 66±18 & 70±13 & 68±18 & 74±20 & 78±11 & 76±12 & 80±15 & 82±14 & 84±15 & 86±16 & 84±15 & 86±16 &  \\
%   & GB = 192 &  40±24 & 54±18 & 72±13 & 84±12 & 92±10 & 88±13 & 88±13 & 92±10 & 94±9 & 92±10 & 98±6 & 94±9 & 94±13 & 98±6 & 98±6 & 98±6 & 100±0 & 96±8  &  \\
%   & GB = 224 &  58±14 & 58±27 & 76±17 & 88±13 & 94±9 & 94±9 & 78±21 & 94±9 & 92±13 & 90±10 & 98±6 & 96±12 & 94±9 & 92±10 & 98±6 & 96±8 & 94±9 & 92±10  &  \\
%   & GB = 256 & 42±14 & 28±20 & 28±20 & 32±16 & 46±20 & 38±17 & 36±17 & 30±20 & 40±15 & 36±28 & 34±24 & 32±26 & 28±22 & 42±26 & 44±23 & 30±18 & 32±22 & 26±18  &  \\

  
% \midrule

% \multirow{3}{*}{Multiple GB}
%   & GB = [0, 160, 192, 224] &  44±27 & 44±17 & 64±23 & 80±13 & 90±10 & 90±10 & 94±9 & 94±9 & 96±8 & 96±8 & 100±0 & 100±0 & 100±0 & 100±0 & 100±0 & 100±0 & 100±0 & 100±0  &  \\
%   & GB = [0, 144, 160, 176, 192, 208, 224, 240] &  26±16 & 58±17 & 66±13 & 82±14 & 90±10 & 92±10 & 94±9 & 94±9 & 94±9 & 94±9 & 94±9 & 94±9 & 94±9 & 94±9 & 94±9 & 94±9 & 94±9 & 94±9  &  \\

%   \midrule

% \multirow{1}{*}{Adaptive GB}
%   & GB = [0, 160, 192, 224] &  44±27 & 60±22 & 78±17 & 86±13 & 92±10 & 90±13 & 88±13 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12  &  \\
% \bottomrule
% \end{tabular}
% %
% }
% \caption{Comparison across different Go Back step sizes and Multiple Go Back step sizes in OGBench Maze Giant.}
% \label{tab:go-back-vs-iterations}
% \end{table}


\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\captionsetup{skip=10pt}
\caption{Comparison across different Go Back step sizes and Multiple Go Back step sizes in OGBench Maze Giant.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccccccccccccccc}
\toprule
\textbf{Method} & \textbf{Variant} & \multicolumn{18}{c}{\textbf{Iterations}} \\
\cmidrule(lr){3-20}
 &  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 15 & 20 & 25 & 30 & 35 & 40 & 45 & 50 \\
\midrule

\multirow{8}{*}{Go Back}
  & GB = 32  & 20±20 & 20±20 & 26±20 & 28±20 & 26±20 & 28±22 & 28±20 & 26±18 & 28±20 & 30±18 & 32±22 & 32±22 & 28±20 & 36±27 & 32±18 & 34±18 & 36±22 & 34±24 \\
  & GB = 64  & 20±20 & 24±22 & 24±20 & 30±22 & 32±24 & 30±22 & 36±23 & 32±24 & 36±23 & 32±20 & 38±26 & 36±25 & 38±21 & 34±22 & 38±26 & 36±25 & 38±26 & 34±22 \\
  & GB = 96  & 20±20 & 26±22 & 28±22 & 30±22 & 28±22 & 34±20 & 36±23 & 38±29 & 30±24 & 36±27 & 42±27 & 42±17 & 46±20 & 46±20 & 44±17 & 46±18 & 48±18 & 46±13 \\
  & GB = 128 & 20±18 & 30±26 & 28±20 & 38±26 & 38±21 & 44±28 & 44±20 & 48±18 & 54±22 & 46±22 & 56±17 & 62±21 & 62±21 & 60±20 & 62±21 & 62±21 & 64±17 & 64±20 \\
  & GB = 160 & 26±22 & 42±23 & 50±22 & 62±21 & 58±17 & 60±18 & 66±18 & 70±13 & 68±18 & 74±20 & 78±11 & 76±12 & 80±15 & 82±14 & 84±15 & 86±16 & 84±15 & 86±16 \\
  & GB = 192 & 40±24 & 54±18 & 72±13 & 84±12 & 92±10 & 88±13 & 88±13 & 92±10 & 94±9  & 92±10 & 98±6  & 94±9  & 94±13 & 98±6  & 98±6  & 98±6  & 100±0 & 96±8  \\
  & GB = 224 & 58±14 & 58±27 & 76±17 & 88±13 & 94±9  & 94±9  & 78±21 & 94±9  & 92±13 & 90±10 & 98±6  & 96±12 & 94±9  & 92±10 & 98±6  & 96±8  & 94±9  & 92±10 \\
  & GB = 256 & 42±14 & 28±20 & 28±20 & 32±16 & 46±20 & 38±17 & 36±17 & 30±20 & 40±15 & 36±28 & 34±24 & 32±26 & 28±22 & 42±26 & 44±23 & 30±18 & 32±22 & 26±18 \\

\midrule

\multirow{3}{*}{Multiple GB}
  & GB = [0,160,192,224]                  & 44±27 & 44±17 & 64±23 & 80±13 & 90±10 & 90±10 & 94±9 & 94±9 & 96±8  & 96±8  & 100±0 & 100±0 & 100±0 & 100±0 & 100±0 & 100±0 & 100±0 & 100±0 \\
  & GB = [0,144,160,176,192,208,224,240] & 26±16 & 58±17 & 66±13 & 82±14 & 90±10 & 92±10 & 94±9 & 94±9 & 94±9  & 94±9  & 94±9  & 94±9  & 94±9  & 94±9  & 94±9  & 94±9  & 94±9  & 94±9 \\

\midrule

\multirow{1}{*}{Adaptive GB}
  & GB = [0,160,192,224] & 44±27 & 60±22 & 78±17 & 86±13 & 92±10 & 90±13 & 88±13 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 & 96±12 \\
\bottomrule
\end{tabular}%
}

\label{tab:go-back-vs-iterations}
\end{table}

==> Tables/OGBench_comparison_baseline.tex <==

% \begin{table}[h]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{l l c c}
% \toprule
% \textbf{Method} & \textbf{Environment} & \textbf{Performance} & \textbf{Inference Time (s)} \\
% \midrule
% \multirow{3}{*}{Diffuser}
%   & maze-medium & 60$\pm$9& 11.84\\
%   & maze-large  & 40 $\pm$ 0& 11.46\\
%   & maze-giant  & 0 $\pm$ 0    & 10.90\\
% \midrule
% \multirow{3}{*}{BoN}& maze-medium & 66 $\pm$ 9& 45.96\\
%   & maze-large  & 40 $\pm$ 0& 48.86\\
%   & maze-giant  & 30 $\pm$ 13 & 94.88 \\
% \midrule
% \multirow{3}{*}{BS}
%   & maze-medium & 94 $\pm$ 9& 15.08\\
%   & maze-large  & 58 $\pm$ 14& 66.16\\
%   & maze-giant  & 32 $\pm$ 24 & 45.20\\
% \midrule
% \multirow{3}{*}{SoP}& maze-medium & 100 $\pm$ 0& 19.18\\
%   & maze-large  & 88$\pm$ 13& 24.76\\
%   & maze-giant  & 62 $\pm$ 23 & 75.54\\
% \midrule
% \multirow{3}{*}{Multi GB (Ours)}& maze-medium & \textbf{100 $\pm$ 0} & 2.38\\
%   & maze-large  & \textbf{100 $\pm$ 0}& 26.28\\
%   & maze-giant  & \textbf{100 $\pm$ 0}& 99.62 \\
% \midrule
% \multirow{3}{*}{Adaptive Terminal (Ours)}
%   & maze-medium & \textbf{100 $\pm$ 0} & 2.66\\
%   & maze-large  & <perf> $\pm$ <std> & <time> \\
%   & maze-giant  & \textbf{100 $\pm$ 0}& 86.12\\
% \bottomrule
% \end{tabular}
% \vspace{0.5em}
% \caption{This table presents the best performance for each baseline. Selections prioritize peak performance, excluding configurations that notably increase inference time without meaningful performance gains.}
% \label{tab:baseline_comparison}
% \end{table}

\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l cc cc cc}
\toprule
\textbf{Method}
  & \multicolumn{2}{c}{\textbf{maze-medium}}
  & \multicolumn{2}{c}{\textbf{maze-large}}
  & \multicolumn{2}{c}{\textbf{maze-giant}} \\
  & Performance & Time (s)
  & Performance & Time (s)
  & Performance & Time (s) \\
\midrule
Diffuser
  & 60$\pm$9   & 11.84 
  & 40$\pm$0   & 11.46 
  & 0$\pm$0    & 10.90 \\
BoN
  & 66$\pm$9   & 45.96 
  & 40$\pm$0   & 48.86 
  & 30$\pm$13  & 94.88 \\
BS
  & 94$\pm$9   & 15.08 
  & 58$\pm$14  & 66.16 
  & 32$\pm$24  & 45.20 \\
SoP
  & 100$\pm$0  & 19.18 
  & 88$\pm$13  & 24.76 
  & 62$\pm$23  & 75.54 \\
% Multi GB (Ours)
%   & \textbf{100$\pm$0} & 2.38  
%   & \textbf{100$\pm$0} & 26.28 
%   & \textbf{100$\pm$0} & 99.62 \\
ABCD (Ours)
  & \textbf{100$\pm$0} & 2.66  
  & \textbf{100$\pm$0}   & 25.04 
  & \textbf{100$\pm$0} & 86.12 \\
\bottomrule
\end{tabular}
\vspace{0.5em}
\caption{This table presents the best performance for each baseline. Selections prioritize peak performance, excluding configurations that notably increase inference time without meaningful performance gains.}
\label{tab:baseline_comparison}
\end{table}

==> Tables/OGBench_comparison_old.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}  % 줄 간격 살짝 늘리기 (선택)
\captionsetup{skip=10pt}  % caption과 표 사이 간격 늘리기

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llccccc}
\toprule
\textbf{Inference Method} & \textbf{Add. Compute} & \textbf{Performance} & \textbf{Inf. Time} & \textbf{NFE} \\
\midrule

\multirow{1}{*}{Diffuser} 
  & T = 256 & 0±0 &  10.90s &  256 &  & \\
  & T = 300 & 0±0  &  13.10s &  300 &  & \\
  & T = 3000 & 0±0  & 120.22s &  3000&  & \\
  & T = 9000 & 0±0  & 352.34s &  9000&  & \\
  

\midrule

\multirow{3}{*}{Best of N} 
  & N = 32 & 2±6 & 12.50s &  256 + 1 &  & \\
  & N = 64 & 2±6 & 13.58s &  256 + 1&  & \\
  & N = 96 & 6±9 & 16.10s &  256 + 1&  & \\
  & N = 128 & 6±9 & 20.50s & 256 + 1 &  & \\
  & N = 160 & 16±15 & 23.60s &  256 + 1&  & \\
  & N = 192 & 18±17 & 31.70s &  256 + 1&  & \\
  & N = 224 & 18±17 & 47.50s &  256 + 1&  & \\
  & N = 256 & 18±17 & 48.76s &  256 + 1&  & \\
  & N = 288 & 18±11 & 56.38s &  (256 + 1) * 4 &  & \\
  & N = 320 & 18±11 & 61.30s &  (256 + 1) * 4 &  & \\
  & N = 352 & 20±13 & 61.50s &  (256 + 1) * 4 &  & \\
  & N = 384 & 20±13 & 61.72s & (256 + 1) * 4 &  & \\
  & N = 416 & 22±14 & 67.10s & (256 + 1) * 4 &  & \\
  & N = 448 & 22±14 & 68.32s & (256 + 1) * 4 &  & \\
  & N = 480 & 20±13 & 69.02s & (256 + 1) * 4 &  & \\
  & N = 512 & 22±14 & 71.80s & (256 + 1) * 4 &  & \\
  & N = 544 & 30±13 & 80.94s & (256 + 1) * 4 &  & \\
  & N = 576 & 30±13 & 85.18s & (256 + 1) * 4 &  & \\
  & N = 608 & 30±13 & 88.66s & (256 + 1) * 4 &  & \\
  
  
  

\midrule

\multirow{4}{*}{Search over Paths}
  & $\Delta f$=200, $\Delta b$=100 & 14±16 & 15.78s & 357 &  & \\
  & $\Delta f$=100, $\Delta b$=50 & 22±11 & 24.06 &  410&  & \\
  & $\Delta f$=50, $\Delta b$=25 & 18±14 & 32.10s &  465&  & \\
  & $\Delta f$=41, $\Delta b$=20 & 28±22 & 35.12s &  478&  & \\
  & $\Delta f$=31, $\Delta b$=15 & 34±24 & 39.42s &  513&  & \\
  & $\Delta f$=21, $\Delta b$=10 & 30±18 & 50.76s &  534&  & \\
  & $\Delta f$=11, $\Delta b$=5 & 20±15 & 77.78s &  601&  & \\
  & $\Delta f$=6, $\Delta b$=3 & 28±16 & 141.74s &  589&  & \\
  & $\Delta f$=4, $\Delta b$=2 & 16±12 & 203.06s &  635&  & \\
  & $\Delta f$=2, $\Delta b$=1 & 20±15 & 380.24s &  765&  & \\

  


\midrule

\multirow{4}{*}{Go Back} 
  & GB = 255, iter = 10 &  36±28&  26.66s &  297&  & \\
  & GB = 224, iter = 10 &  90±10&  26.02s& 267 &  & \\
  & GB = 192, iter = 10 &  92±10&  24.12s&  237&  & \\
  & GB = 160, iter = 10 &  74±20&  22.38s&  207&  & \\
  & GB = 128, iter = 10 &  46±22&  21.82s&  167&  & \\
  & GB = 96, iter = 10 &  36±27&  21.32s& 137 &  & \\
  & GB = 64, iter = 10 &  32±20&  19.54s& 107 &  & \\
  & GB = 32, iter = 10 &  30±18&  18.22s&  77&  & \\
\midrule



\multirow{1}{*}{\shortstack[l]{Multiple Go Back}}
  & iteration 15  &  100±0 &  37.34s& 387 & &\\
  
\midrule

% \multirow{1}{*}{\shortstack[l]{Adaptive Go Back}}
%   & 10 even, iter =  55  &  &  &  & &\\
%   & 5 even, iter = 55  &  &  &  & &\\
%   & 3 even, iter = 55  &  &  &  & &\\
  
% \midrule

\multirow{1}{*}{\shortstack[l]{Adaptive thinking}} 
  & max iteration 15  & 100±0 &  36.9s&  < 387& &\\


\bottomrule
\end{tabular*}
\caption{Comparison of various inference-time strategies across compute and performance in OGBench Maze Giant.}
\label{tab:adaptive-diffusion-results}
\end{table}

==> Tables/PixelMaze_GoBack_comparison.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\captionsetup{skip=10pt}  % 캡션과 테이블 사이 간격 조절

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llcccccc}
\toprule
\textbf{Method} & \textbf{Variant} & \multicolumn{6}{c}{\textbf{Iterations}} \\
\cmidrule(lr){3-8}
& & \textbf{1} & \textbf{5} & \textbf{10} & \textbf{15} & \textbf{20} & \textbf{25} \\
\midrule

\multirow{4}{*}{Go Back}
  & GB = 10 & 0.07 & 0.12 & 0.10 & 0.13 & 0.18 & 0.23 \\
  & GB = 20 & 0.08 & 0.11 & 0.24 & 0.27 & 0.46 & 0.55 \\
  & GB = 30 & 0.16 & 0.37 & 0.73 & 0.86 & 0.96 & 0.94 \\
  & GB = 40 & 0.19 & 0.92 & 0.97 & 1.00 & 0.98 & 0.98 \\

\midrule

\multirow{3}{*}{Multiple GB}
  & 10 even & 0.17 & 0.68 & 0.97 & 0.99 & 0.97 & 0.99 \\
  & 5 even & 0.14 & 0.62 & 0.9 & 0.95 & 0.96 & 0.96 \\ 
  & Best 2[30,40] & 0.18 & 0.89 & 0.99 & 0.99 & 0.97 & 0.99 \\
  
\midrule

\multirow{3}{*}{Adaptive GB}
  & 10 even &  &  &  &  &  &  \\
  & 5 even &  &  &  &  &  &  \\
  & 3 even &  &  &  &  &  &  \\

\bottomrule
\end{tabular*}
\caption{Comparison across different Go Back strategies in Pixel Maze setting over iterations.}
\label{tab:go-back-vs-iterations}
\end{table}

==> Tables/PixelMaze_multiSize_comparison.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\captionsetup{skip=10pt}

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lllccc}
\toprule
\textbf{Maze Size} & \textbf{Method} & \textbf{Variant} & \textbf{Performance (\%)} & \textbf{Inference Time (s)} \\
\midrule

\multirow{5}{*}{\centering 11}
   &                   & N = 20 &  & s & \\
   & Best of N         & N = 40 &  & s &  \\
   &                   & N = 80 &  & s & \\
   &                   & $\Delta f = 40$, $\Delta b = 20$  & 0.84 ± 0.36 & 2.24s & \\
   & Search over Paths & $\Delta f = 20$, $\Delta b = 10$ & 0.97 ± 0.17 & 2.86s & \\
   &                   & $\Delta f = 10$, $\Delta b = 5$ & \textbf{1.0} ± 0.0 & 3.84s & \\
   & Adaptive Thinking &  stop flag = 3   & \textbf{1.0} & \textbf{1.71s} & \\
\midrule

\multirow{5}{*}{\centering 12}
   &                   & N = 20 &  & s & \\
   & Best of N         & N = 40 &  & s &  \\
   &                   & N = 80 &  & s & \\
   &                   & $\Delta f = 40$, $\Delta b = 20$ & 0.8 ± 0.4 & 2.79s & \\
   & Search over Paths & $\Delta f = 20$, $\Delta b = 10$ & 0.92 ± 0.27 & 3.50s & \\
   &                   & $\Delta f = 10$, $\Delta b = 5$ & \textbf{0.99 ± 0.09} & 4.44s & \\
   & Adaptive Thinking & stop flag = 3    & \textbf{1.0} & \textbf{2.11s} & \\
\midrule

\multirow{5}{*}{\centering 13}
   &                   & N = 20 &  & s & \\
   & Best of N         & N = 40 &  & s &  \\
   &                   & N = 80 &  & s & \\
   &                   & $\Delta f = 40$, $\Delta b = 20$  & 0.48 ± 0.49 & 3.21s & \\
   &                   & $\Delta f = 20$, $\Delta b = 10$ & 0.86 ± 0.34 & 4.02s & \\
   & Search over Paths & $\Delta f = 10$, $\Delta b = 5$ & 0.95 ± 0.21 & 5.26s & \\
   &                   & $\Delta f = 8$, $\Delta b = 4$ & 0.97 ± 0.17 & 5.44s & \\
   &                   & $\Delta f = 4$, $\Delta b = 2$ & \textbf{0.97 ± 0.17} & 7.28s & \\
   & Adaptive Thinking & stop flag = 3    & \textbf{0.99} & \textbf{2.88s} & \\
\midrule

\multirow{5}{*}{\centering 14}
   &                   & $p = 3$ & 0.41 & 3.97s & \\
   & BS                & $p = 2$ & 0.47 & 5.54s &  \\
   &                   & $p = 1$ & 0.68 & 10.18s & \\
   &                   & $\Delta f = 40$, $\Delta b = 20$  & 0.42 ± 0.49 & 3.58s & \\
   &                   & $\Delta f = 20$, $\Delta b = 10$ & 0.66 ± 0.47 & 4.43s & \\
   & Search over Paths & $\Delta f = 10$, $\Delta b = 5$ & 0.8 ± 0.4 & 5.60s & \\
   &                   & $\Delta f = 8$, $\Delta b = 4$ & 0.9 ± 0.3 & 5.86s & \\
   &                   & $\Delta f = 6$, $\Delta b = 3$ & \textbf{0.97 ± 0.17} & 6.45s & \\
   & Adaptive Thinking & stop flag = 3    & \textbf{1.0} & \textbf{3.27s} & \\
\midrule

\multirow{5}{*}{\centering 15}
   &                   & $p = 2$ &  & s & \\
   & SMC               & $p = 1$ &  & s &  \\
   &                   & $p = 1$ &  & s &  \\
   &  Beam Search      & $p = 2$ & 0.39 & 5.69s & \\
   &                   & $p = 1$ & 0.52 & 10.65s & \\
   &                   & $\Delta f = 40$, $\Delta b = 20$ & 0.25 ± 0.43 & 4.05s &  \\
   &                   & $\Delta f = 20$, $\Delta b = 10$ & 0.54 ± 0.49 & 4.98s &  \\
   &                   & $\Delta f = 10$, $\Delta b = 5$ & 0.76 ± 0.42 & 6.35s &  \\
   & SoP                  & $\Delta f = 8$, $\Delta b = 4$ & 0.85 ± 0.35 & 6.69s & \\
   &  & $\Delta f = 6$, $\Delta b = 3$ & 0.91 ± 0.28 & 7.08s & \\
   &                   & $\Delta f = 4$, $\Delta b = 2$ & 0.95 ± 0.21 &  8.43s & \\
   &                   & $\Delta f = 2$, $\Delta b = 1$ & 0.98 ± 0.13 & 12.42s & \\
   %&                   & $p = 5$ & 0.22 &  2.67s & \\
   %&                   & $p = 4$ & 0.28 & 3.25s & \\
   %& Beam Search       & $p = 3$ & 0.27 &  4.13s & \\
   & Adaptive Thinking & stop flag = 3    & \textbf{0.99} & \textbf{4.17s} & \\
\bottomrule
\end{tabular*}
\caption{Comparison of Search over Paths and Adaptive Thinking across maze sizes.}
\label{tab:maze-method-comparison}
\end{table}

==> Tables/Sudoku_GoBack_comparision.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\captionsetup{skip=10pt}  % 캡션과 테이블 사이 간격 조절

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llcccccccccccc}
\toprule
\textbf{Method} & \textbf{Variant} & \multicolumn{12}{c}{\textbf{Iterations}} \\
\cmidrule(lr){3-14}
 &  & 1 & 5 & 10 & 15 & 20 & 25 & 30 & 35 & 40 & 45 & 50 & 55 \\
\midrule

\multirow{4}{*}{Go Back}
  & GB = 10 & 0.57 & 0.61 & 0.64 & 0.65 & 0.67 & 0.67 & 0.67 & 0.69 & 0.69 & 0.67 & 0.70 & 0.70 \\
  & GB = 20 & 0.6 & 0.73 & 0.83 & 0.88 & 0.94 & 0.96 & 0.98 & 0.98 & 0.99 & 0.99 & 0.99 & 0.99 \\
  & GB = 30 & 0.62 & 0.80 & 0.87 & 0.90 & 0.91 & 0.91 & 0.91 & 0.91 & 0.91 & 0.91 & 0.92 & 0.91  \\
  & GB = 40 & 0.63 & 0.70 & 0.69 & 0.69 & 0.69 & 0.69 & 0.69 & 0.7 & 0.69 & 0.69 & 0.69 & 0.70 \\

\midrule

\multirow{3}{*}{Multiple GB}
  & 10 even & 0.60 & 0.77 & 0.88 & 0.92 & 0.95 & 0.97 & 0.98 & 0.98 & 0.98 & 0.99 & 0.99 & 0.99 \\
  & 5 even &  0.60 & 0.79 & 0.89 & 0.94 & 0.97 & 0.97 & 0.98 & 0.99 & 0.98 & 0.99 & 0.99 & 0.99 \\
  & 3 even & 0.59 & 0.8 & 0.90 & 0.93 & 0.96 & 0.97 & 0.98 & 0.99 & 0.99 & 0.99 &  0.99 & 0.99 \\
  & Best 2 [20,30] & 0.61 & 0.79 & 0.90 & 0.95 & 0.97 & 0.98 & 0.99 & 0.99 & 1.0 & 0.98 &  1.0 & 0.99 \\
  
\bottomrule


\multirow{3}{*}{Adaptive GB}
  & 10 even &  &  &  &  &  &  &  &  &  &  &  &  \\
  & 5 even &  &  &  &  &  &  &  &  &  &  &  &  \\
  & 3 even &  &  &  &  &  &  &  &  &  &  &  &  \\
  
\bottomrule
\end{tabular*}
\caption{Comparison across different Go Back step size and Multiple Go Back step size in Sudoku setting.}
\label{tab:go-back-vs-iterations}
\end{table}

==> Tables/Sudoku_comparison.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}  % 줄 간격 살짝 늘리기 (선택)
\captionsetup{skip=10pt}  % caption과 표 사이 간격 늘리기

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llccccc}
\toprule
\textbf{Inference Method} & \textbf{Add. Compute} & \textbf{Performance} & \textbf{Inf. Time} & \textbf{NFE} \\
\midrule

\multirow{1}{*}{Standard Diffusion} 
  & No add & 0.4 ± 0.12 &  0.62s &  &  & \\

\midrule

\multirow{3}{*}{Best of N} 
  & N = 40 & 0.60 ± 0.12 & 0.62s &  &  & \\
  & N = 80 & 0.64 ± 0.13 & 0.61s &  &  & \\
  & N = 120 & 0.65 ± 0.13 & 0.62s &  &  & \\
  & N = 240 & 0.68 ± 0.12 & 0.74s &  &  & \\
  & N = 480 & 0.7 ± 0.12  & 1.02s &  &  & \\
  & N = 960 & 0.72 ± 0.12 & 1.68s &  &  & \\
  & N = 1920 & 0.73 ± 0.12 & 3.26s &  &  & \\
  & N = 3840 & 0.75 ± 0.12 & 6.07s &  &  & \\

\midrule

\multirow{4}{*}{Search over Paths}
  & $\Delta f$=10, $\Delta b$=5 & 0.77 ± 0.13 & 0.86s &  &  & \\
  & $\Delta f$=8, $\Delta b$=4 & 0.78± 0.12 & 0.85s &  &  & \\
  & $\Delta f$=6, $\Delta b$=3 & 0.80 ± 0.12  & 0.89s &  &  & \\
  & $\Delta f$=4, $\Delta b$=2 & 0.82 ± 0.12  & 0.87s &  &  & \\
  & N = 120, $\Delta f$=4, $\Delta b$=2 & 0.89 ± 0.1  & 1.73s &  &  & \\
  & N = 200, $\Delta f$=4, $\Delta b$=2 & 0.90 ± 0.1  & 2.61s &  &  & \\
  & N = 250, $\Delta f$=4, $\Delta b$=2 & 0.90 ± 0.09  & 3.26s &  &  & \\
  

\midrule

\multirow{4}{*}{Go Back} 
  & GB = 10, iter = 55 & 0.704 ± 0.13  & 0.94s &  &  & \\
  & GB = 20, iter = 55 & 0.998 ± 0.01 & 1.39s &  &  & \\
  & GB = 30, iter = 55 & 0.918  ± 0.11 & 1.88s &  &  & \\
  & GB = 40, iter = 55 & 0.703 ± 0.14 & 2.27s &  &  & \\
  
\midrule

\multirow{1}{*}{\shortstack[l]{Multiple Go Back}}
  & 10 even, iter =  55  & 0.996 ± 0.01 & 2.5s &  & &\\
  & 5 even, iter = 55  & 0.999 ± 0.005 & 2.45s &  & &\\
  & 3 even, iter = 55  & 0.996 ± 0.01 & 2.80s &  & &\\
  
\midrule

\multirow{1}{*}{\shortstack[l]{Adaptive thinking}} 
  & 10 even, max iter 100, sf = 5  & 0.992 ± 0.02 & 1.43s &  &  & \\
  & 10 even, max iter 100, sf = 10  & 0.997 ± 0.014 & 1.62s &  &  & \\
  & 10 even, max iter 100, sf = 20  & \textbf{0.999 ± 0.006} & 2.07s &  &  & \\
  & 5 even, max iter 100, sf = 5  & 0.981 ± 0.05 & 1.25s &  &  & \\
  & 5 even, max iter 100, sf = 10  & 0.995 ± 0.02 & 1.51s &  &  & \\
  & 5 even, max iter 100, sf = 20  & \textbf{0.999 ± 0.005} & 2.10s &  &  & \\

\midrule

\multirow{1}{*}{\shortstack[l]{Adaptive Go Back}}
  & 10 even, iter =  55  &  &  &  & &\\
  & 5 even, iter = 55  &  &  &  & &\\
  & 3 even, iter = 55  &  &  &  & &\\


\bottomrule
\end{tabular*}
\caption{Comparison of various inference-time strategies across compute and performance in Sudoku setting.}
\label{tab:adaptive-diffusion-results}
\end{table}

==> Tables/TextToImage_aesthetic_old.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}  % 줄 간격 살짝 늘리기 (선택)
\captionsetup{skip=10pt}  % caption과 표 사이 간격 늘리기
\caption{Comparison of various inference-time strategies across compute and aesthetic score in the Text-to-image generation task.}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llccccc}
\toprule
\textbf{Inference Method} & \textbf{Add. Compute} & \textbf{Image Aesthetic} & \textbf{Inference wall clock time (sec.)} %& \textbf{NFE}  
\\
\midrule

\multirow{1}{*}{Base Diffusion} 
  & No add & 5.57 ± 0.03 & 58.83 &  &  & \\

\midrule

\multirow{3}{*}{} 
  & N = 2 & 5.63 ± 0.08 & 109.75 &  &  & \\
  & N = 3 & 5.72 ± 0.09 & 150.92 &  &  & \\
  & N = 4 & 5.75 ± 0.07 & 200.58 &  &  & \\
  & N = 5 & 5.79 ± 0.05 & 258.33 &  &  & \\
  & N = 6 & 5.81 ± 0.02 & 293.42 &  &  & \\
  BoN & N = 7 & 5.81 ± 0.02 & 349.00 &  &  & \\
  & N = 8 & 5.82 ± 0.03 & 403.50 &  &  & \\
  & N = 9 & 5.86 ± 0.05 & 445.25 &  &  & \\
  & N = 10 & 5.86 ± 0.05 & 494.25 &  &  & \\
  & N = 11 & 5.87 ± 0.04 & 556.75 &  &  & \\
  & N = 12 & 5.90 ± 0.05 & 583.17 &  &  & \\

\midrule

\multirow{4}{*}{}
   & $\Delta f = 500$, $\Delta b = 250$ & 5.76 ± 0.05 & 182.00 &  \\
    & $\Delta f = 400$, $\Delta b = 200$ & 5.78 ± 0.03 & 207.67 &  \\
  SoP & $\Delta f = 300$, $\Delta b = 150$ & 5.81 ± 0.01 & 241.75 &  \\
    & $\Delta f = 200$, $\Delta b = 100$ & 5.83 ± 0.09 & 262.00 & \\
    & $\Delta f = 100$, $\Delta b = 50$ & 5.93 ± 0.10 & 299.92 & \\

\midrule

\multirow{1}{*}{\shortstack[l]{}} 
  & \texttt{max\_iter} = 10  & 5.96 ± 0.06 & 27.00 &  & &\\
  & \texttt{max\_iter} = 20 & 5.99 ± 0.06 & 43.33 &  & &\\
  ABCD & \texttt{max\_iter} = 30 & 6.04 ± 0.09 & 60.00 &  & &\\
   & \texttt{max\_iter} = 40 & 6.06 ± 0.08 & 79.17 &  & &\\
  & \texttt{max\_iter} = 50 & 6.10 ± 0.07 & 95.67 &  & &\\
  & \texttt{max\_iter} = 80 & 6.14 ± 0.07 & 143.08 &  & &\\

  
\bottomrule
\end{tabular*}


\label{tab:text2img_aesthetic_main_results}
\end{table}

==> Tables/TextToImage_hps_old.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}  % 줄 간격 살짝 늘리기 (선택)
\captionsetup{skip=10pt}  % caption과 표 사이 간격 늘리기
\caption{Comparison of various inference-time strategies across compute and human preference score in the Text-to-image generation task.}
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llccccc}
% \toprule
% \textbf{Inference Method} & \textbf{Add. Compute} & \textbf{Human Preference} & \textbf{Inference wall clock time (sec.)} & \textbf{NFEs}  
% \\
% \midrule

% \multirow{1}{*}{Base Diffusion} 
%   & No add & 0.2710 ± 0.0028 & 61.00 &  &  & \\

% \midrule

% \multirow{3}{*}{} 
%   & N = 2 & 0.2749 ± 0.0013 & 112.25 &  &  & \\
%   BoN & N = 3 & 0.2752 ± 0.0017 & 153.00 &  &  & \\
%   & N = 4 & 0.2752 ± 0.0018 & 203.08 &  &  & \\
%   & N = 5 & 0.2753 ± 0.0017 & 260.92 &  &  & \\

% \midrule

% \multirow{4}{*}{}
%    & $\Delta f = 500$, $\Delta b = 250$ & 0.2722 ± 0.0035 & 184.42 &  \\
%     & $\Delta f = 400$, $\Delta b = 200$ & 0.2746 ± 0.0022 & 209.83 &  \\
%   SoP & $\Delta f = 300$, $\Delta b = 150$ & 0.2744 ± 0.0041 & 244.42 &  \\
%     & $\Delta f = 200$, $\Delta b = 100$ & 0.2746 ± 0.0045 & 265.08 & \\
%     & $\Delta f = 100$, $\Delta b = 50$ & 0.2764 ± 0.0046 & 304.92 & \\

% \midrule

% \multirow{1}{*}{\shortstack[l]{}} 
%   & \texttt{max\_iter} = 10  & 0.2741 ± 0.0022 & 28.42 &  & &\\
%   & \texttt{max\_iter} = 20 & 0.2756 ± 0.0019 & 44.83 &  & &\\
%   ABCD & \texttt{max\_iter} = 30 & 0.2763 ± 0.0014 & 61.75 &  & &\\
%    & \texttt{max\_iter} = 40 & 0.2770 ± 0.0018 & 80.75 &  & &\\
%   & \texttt{max\_iter} = 50 & 0.2774 ± 0.0016 & 95.92 &  & &\\
%   & \texttt{max\_iter} = 80 & 0.2786 ± 0.0029 & 141.75 &  & &\\
  
% \bottomrule
% \end{tabular*}

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llccccc}
\toprule
\textbf{Inference Method} & \textbf{Add. Compute} & \textbf{Human Preference} & \textbf{Clock time (sec.)} & \textbf{NFEs}  
\\
\midrule

\multirow{1}{*}{Base Diffusion} 
  & No add & 0.2710 ± 0.0028 & 61.00 & 2000 &  & \\

\midrule

\multirow{4}{*}{BoN} 
  & N = 2 & 0.2749 ± 0.0013 & 112.25 & 4000 &  & \\
  & N = 3 & 0.2752 ± 0.0017 & 153.00 & 6000 &  & \\
  & N = 4 & 0.2752 ± 0.0018 & 203.08 & 8000 &  & \\
  & N = 5 & 0.2753 ± 0.0017 & 260.92 & 10000 &  & \\

\midrule

\multirow{7}{*}{SoP}
   & $\Delta f = 510$, $\Delta b = 255$ & 0.2725 ± 0.0031 & 192.83 & 7548 &  \\
    & $\Delta f = 410$, $\Delta b = 205$ & 0.2728 ± 0.0030 & 221.00 & 8490 & \\
  & $\Delta f = 350$, $\Delta b = 175$ & 0.2739 ± 0.0044 & 233.00 & 9192 & \\
    & $\Delta f = 230$, $\Delta b = 115$ & 0.2751 ± 0.0029 & 272.25 & 10218 & \\
    & $\Delta f = 130$, $\Delta b = 65$ & 0.2765 ± 0.0046 & 811.25 & 11232 &\\
    & $\Delta f = 70$, $\Delta b = 35$ & 0.2777 ± 0.0039 & 335.42 & 11778 & \\
    & $\Delta f = 20$, $\Delta b = 10$ & 0.2787 ± 0.0027 & 431.42 & 13056 &\\

\midrule

\multirow{8}{*} {ABCD}%{\shortstack[l]{}} 
  & \texttt{max\_iter} = 10  & 0.2776 ± 0.0027 & 46.83 & 1280 & &\\
  & \texttt{max\_iter} = 20 & 0.2791 ± 0.0021 & 82.83 & 2260 & &\\
  & \texttt{max\_iter} = 30 & 0.2797 ± 0.0023 & 115.92 & 3240 & &\\
   & \texttt{max\_iter} = 40 & 0.2804 ± 0.0027 & 142.17 & 4220 & &\\
  & \texttt{max\_iter} = 50 & 0.2808 ± 0.0028 & 183.42 & 5200 & &\\
  & \texttt{max\_iter} = 80 & 0.2815 ± 0.0030 & 272.08 & 7960 & &\\
  & \texttt{max\_iter} = 100 & 0.2819 ± 0.0032 & 322.08 & 9618 & &\\
  & \texttt{max\_iter} = 200 & 0.2823 ± 0.0033 & 432.92 & 12616 & &\\


\bottomrule
\end{tabular*}


\label{tab:text2img_hps_main_results}
\end{table}
